Spotlight the Negatives: A Generalized Discriminative Latent Model

Discriminative latent variable models (LVM) are frequently applied to various visual recognition tasks. In these systems the latent (hidden) variables provide a formalism for modeling structured variation of visual features. Conventionally, latent variables are de- fined on the variation of the foreground (positive) class. In this work we augment LVMs to include negative latent variables corresponding to the background class. We formalize the scoring function of such a generalized LVM (GLVM). Then we discuss a framework for learning a model based on the GLVM scoring function. We theoretically showcase how some of the current visual recognition methods can benefit from this generalization. Finally, we experiment on a generalized form of Deformable Part Models with negative latent variables and show significant improvements on two different detection tasks.

==> DPM_full.tex <==
\section{Deformable Part Models}
\label{sec:dpm}
Part based models have had a long and successful presence in the history of Computer Vision \cite{CootesET99, LeibeLS08, BourdevM09, ZhuCY10, FelzenszwalbMR08}.

Deformable Part Models (DPMs)~\cite{FelzenszwalbMR08} have been extensively used for object detection over the past decade. Despite their incredible flexibility to object deformation and viewpoint changes they only look for positive evidence in images. In particular, DPMs do not capture counter evidence. For example, the knowledge that a cow-head detector fires strongly on a detection window should decrease the score of  horse-detector on that window. We propose an extension to DPMs by augmenting them with negative parts. We call our model \emph{Generalized-DPM} (or GDPM in short).

Training of the proposed model does not fit in the latent SVM framework~\cite{FelzenszwalbMR08}. We propose an algorithm to learn DPMs with negative parts. Our experimental results show that negative parts complement DPMs~\cite{FelzenszwalbMR08}.
DPM is a mixture of multi-scale part-based object detectors. Each mixture component captures appearance of the object in a specific viewpoint. Each mixture has a \emph{root} filter for capturing the global structure of the object in a coarse scale. It also has a set of \emph{deformable part} filters for capturing parts of the object individually in a higher resolution. DPM uses sliding window search to detect objects. The root filter is used as the detection window during training. Consider a DPM with $\cntPartsPos$ parts. We denote the location (and size) of the root filter and the parts by $\rootLocation$ and $l=(l_1, \dots, l_\cntPartsPos)$ respectively. We also denote the choice of the mixture component by $c$. The true root, and part locations as well as the choice of the mixture component are unknown even during training and, therefore, are treated as latent variables in a DPM. 

We define a \emph{latent configuration} as an assignment of all latent variables in the model and denote it by $z=(c, \rootLocation, l)$. Score of a DPM with latent configuration $z$ on image $x$ is a linear function of the model parameters, which we denote by $\beta$, and is defined as follows:
\begin{align}
	g_\beta(x, z) = \beta \cdot \Phi(x, z)
	\label{eq:score_config_dpm}
\end{align}
where $\Phi(x, z)$ extracts features from image $x$ according to the latent configuration $z$.

\iffalse
DPM is a mixture model where each mixture component captures appearance of the object in a specific viewpoint. We denote a DPM with $\cntMixtures$ mixture components by $\beta=(\beta_1; \dots; \beta_\cntMixtures)$. Each mixture component $\beta_c=(F_{c, 0}; w_{c, 1}; \dots; w_{c, \cntPartsPos})$ is parameterized by a root filter $F_{c, 0}$, and $\cntPartsPos$ parts where each part $w_{c, j}=(F_{c, j}; d_{c, j})$ has an appearance model $F_{c, j}$ and a deformation model $d_{c, j}$.

Let $\rootLocation$ denote the location (and size) of root filter and let $z=(c, l_1, \dots, l_\cntPartsPos)$ denote a latent configuration that includes the choice of the mixture component $c$ and location (and size) of all the parts $l_1, \dots, l_\cntPartsPos$. For each part $l_j \in L_j(x)$ where $L_j(x)$ denotes the set of all valid placements of part $j$ on image $x$. Score of a DPM $\beta$ with latent configuration $z$ on image $x$ is a linear function of the model parameters $\beta$ and is defined as follows:
\begin{align}
	f_\beta(x, \rootLocation, z) = \beta \cdot \Phi(x, \rootLocation, z)
	\label{eq:score_roots_dpm}
\end{align}
where $\Phi(x, \rootLocation, z)$ extracts features from image $x$ at detection window $\rootLocation$ according to the latent configuration $z$.
\fi

Let $R$ be a set of candidate root locations (for examples, all detection windows that have high overlap with a given image region). We denote the detection score on $R$ by $f_\beta(x, R)$ and define it as the score of the best latent configuration that places the root filter at a location in $R$ as follows:
\begin{align}
	f_\beta(x, R) = \max_{\substack{z=(\rootLocation, c, l) \\ \text{\st $\rootLocation \in R$}}} g_\beta(x, z)
	\label{eq:score_roots_dpm}
\end{align}

\iffalse
\todo{mention that DPM is parameterized as such and such}
Part dependencies in the standard DPM respect a star configuration with the root filter at the center of the star. Thus, part locations are independent given the location of the root filter. Let $\phi_a(x, l_j)$ denote appearance features extracted from patch $l_j$ of image $x$ (\eg HOG features). Also let $\phi_d(l_j, \rootLocation)$ denote the deformation features of placing part $j$ at $l_j$ given that the root filter is placed at $\rootLocation$. We define the feature function $\phi(x, l_j, \rootLocation)=( \phi_a(x, l_j); \phi_d(l_j, \rootLocation) )$. For DPMs, we can rewrite Equation~\ref{eq:score_roots_dpm} as follows:
\begin{align}
	f_\beta(x, R) &= \max_{\rootLocation \in R} \max_c F_{c, 0} \cdot \phi_a(x, \rootLocation) \notag \\
		& \hspace{0.75cm} + \sum_{j=1}^\cntPartsPos \max_{l_j} w_{c, j} \cdot \phi(x, l_j, \rootLocation) \label{eq:score_roots_dpm_expanded}
\end{align}
\fi

\subsection{Training Deformable Part Models}
Let $\mathcal{D} = \{ (x_i, y_i, b_i) \}_{i=1}^\cntAnnotations$ denote a set of $\cntAnnotations$ annotated training examples. $x_i$ denotes an image. $y_i \in \{+1, -1\}$ denotes a class label that determines whether the example is foreground ($y_i = +1$) or background ($y_i = -1$). $b_i$ denotes the coordinates of the annotated bounding box that circumscribes the object in a foreground image. $b_i$ is irrelevant if $y_i=-1$. All root filter locations on a background image are considered as independent negative examples. 

DPM uses the root filter as a detection window during training. Despite availability of $b_i$'s for foreground images, DPM treats true detection bounding boxes on the foreground images as latent variables. Any root filter whose overlap with the annotated bounding box $b_i$ exceeds a certain threshold $\tau$ is considered as a valid detection (true positive) for $b_i$. We denote the set of valid detections of $b_i$ by $H(x_i, b_i, \tau)$. In order to train DPMs a separate training set $D=\{ (x_i, y_i, R_i) \}_{i=1}^\cntExamples$ is constructed from the annotated examples in $\mathcal{D}$. Each background example $(x, y=-1, b_i) \in \mathcal{D}$ adds multiple examples $(x, y, \{\rootLocation\})$ to $D$, one for each root placement $\rootLocation$. Each foreground example $(x, y=+1, b_i) \in \mathcal{D}$ adds one example $(x, y, R)$ to $D$ where $R=H(x, b, \tau)$. In DPM, the value of $\tau$ is set to $0.7$.

DPM uses Latent SVM~\cite{FelzenszwalbMR08} for training. Given the training set $D$, the model parameters $\beta$ are trained by minimizing the following objective function:
\begin{align}
	O(\beta) = \frac{1}{2} ||\beta||^2 + C \sum_{i=1}^\cntExamples \max \{ 0, 1 - y_i f_\beta(x_i, R_i) \}
	\label{eq:of_dpm}
\end{align}
The objective function in Equation~\ref{eq:of_dpm} is non-convex. Particularly, $f_\beta(x_i, R_i)$ as defined in Equation \ref{eq:score_roots_dpm} is maximum of a set of linear functions $g_\beta(x, z)$, and therefore is convex. Then for samples with $y>0$ the hinge loss in Equation \ref{eq:of_dpm} becomes concave. \\
Latent SVM employs an alternating approach similar to CCCP~\cite{YuilleR03} to minimize the training objective. CCCP is an iterative procedure that alternates between 1) constructing a convex upper bound on the original objective function and 2) optimizing the bound. CCCP is guaranteed to converge to a local minimum of the original objective function. 

In the case of DPMs, the first step boils down to fixing the value of the latent variables in Equation \ref{eq:of_dpm} for \emph{foreground} examples. Let $z_i=(\rootLocation_i, c_i, l_{i, 1}, \dots, l_{i, n})$ denote a particular assignment of the latent variables for the foreground example $(x_i, y_i, R_i)$. A convex upper bound to $O(\beta)$ is defined as follows:
\begin{align}
	B(\beta) =& \frac{1}{2} ||\beta||^2 + C \sum_{\substack{i=1 \\ y_i=-1}}^\cntExamples \max \{ 0, 1 + f_\beta(x_i, R_i) \} \notag \\
	& \hspace{0.9cm} + C \sum_{\substack{i=1 \\ y_i=+1}}^\cntExamples \max \{ 0, 1 - g_\beta(x_i, z_i) \}
	\label{eq:bound_dpm}
\end{align}
We call this the \emph{relabeling} step of the training algorithm.

The second step involves solving the following optimization problem:
\begin{align}
	\beta^* = \argmin_\beta B(\beta)
\end{align}
Any assignment of $z_i$'s for foreground examples leads to a convex function (Equation~\ref{eq:bound_dpm}) which is an upper bound to $O$ (Equation~\ref{eq:of_dpm}). In order to guarantee progress in each iteration we require that $z_i$'s are set to the maximum scoring configurations under the previous model $\beta^*$ as follows:
\begin{align}
	z_i=\argmax_z g_{\beta^*}(x_i, z), \; \forall i \;\st \; y_i=+1
\end{align}

%-------------------------------------------------------------------------
\subsection{Negative Parts}
In a binary classifier, a negative (positive) part is defined as a part whose \emph{maximum} response is \emph{subtracted} from (\emph{added} to) the classification score~\cite{PariziVZF15}. 
%\todo{elaborate more on the definition of negative parts}

While positive parts collect evidence for presence of an object negative parts collect \emph{counter-evidence} for it. For example, consider a detection window $\omega$. Presence of a \emph{saddle} in the detection window $\omega$ should decrease the score of a \emph{cow} detector on $\omega$. This is because \emph{cow}s tend not to have \emph{saddle}s on their backs. Thus, if we find a \emph{saddle} in the detection window of a \emph{cow} detector we, most likely, are confusing a \emph{horse} for a \emph{cow}. Counter evidence is particularly important in discriminating between similar objects; like \emph{cow} from \emph{horse} in the hypothetical example above. We obtain this behavior by augmenting \emph{cow} detector model with a negative part that fires on \emph{saddle}.

Finally, we note that standard DPMs cannot capture counter-evidence. For example, if $F$ is the appearance model of a positive part, $-F$ does \emph{not} make it a negative part. In this paper we extend DPMs by augmenting them with negative parts.

%\todo{maybe add a mathematical definition?}

%-------------------------------------------------------------------------
\subsection{Adding Negative Parts to Deformable Part Models}
In DPM, responses of all part filters are \emph{added} to the detection score of the classifier. Thus, DPMs cannot model negative parts. We generalize DPMs by augmenting them with negative parts. We call the proposed model \emph{Generalized-DPM} (or GDPM in short). Standard DPM~\cite{FelzenszwalbMR08} is a GDPM with zero negative parts.

\noindent We denote a GDPM with $\cntMixtures$ mixture components by $\gamma=(\gamma_1; \dots; \gamma_\cntMixtures)$. 
Each mixture component captures the appearance of the object in a viewpoint. A mixture component with $\cntPartsPos$ positive parts and $\cntPartsNeg$ negative parts is parameterized by $\gamma_c = (F_{c, 0}; w^+_{c , 1}; \dots; w^+_{c, \cntPartsPos}; w^-_{c, 1}; \dots; w^-_{c, \cntPartsNeg})$. $F_{c, 0}$ denotes the root filter, $w^+_j$'s denote the positive part models, and $w^-_j$'s denote the negative part models. Each part model $w_{c, j} = (F_{c, j}; d_{c, j})$ has an appearance $F_{c, j}$ and a deformation parameter vector $d_{c, j}$.

Let $l^+=(l^+_1, \dots, l^+_\cntPartsPos)$ denote the positive part placements and $l^-=(l^-_1, \dots, l^-_\cntPartsNeg)$ denote the negative part placements. We denote a latent configuration in a GDPM by $z=(\rootLocation, c, l^+, l^-)$. Score of a GDPM $\gamma$ with latent configuration $z$ on image $x$ is a linear function of the model parameters $\gamma$. We denote this by $g_\gamma(x, z)$ and define it as follows:
\begin{align}
	g_\gamma(x, z) = \gamma \cdot \Phi(x, z)
	\label{eq:score_config_gdpm}
\end{align}
where $\Phi$ extracts features from image $x$ according to the latent configuration $z$. This is very similar to the score function of the standard DPM (see Equation~\ref{eq:score_config_dpm}). For example, both functions are linear in the model parameters. Detection score of placing the root at $\rootLocation$, however, is fundamentally different for the two models. For example, unlike Equation~\ref{eq:score_roots_dpm} we \emph{cannot} compute $f_\gamma(x, R)$ by maximizing over all the latent variables. We will elaborate more on the differences between $f_\beta(x, R)$ and $f_\gamma(x, R)$ in the rest of this section. 

Like in DPM, part dependencies in GDPM respect a star configuration with the root filter at the center of the star. Thus, part placements are independent given the location of the root filter. Let $\phi_a(x, l_j)$ denote appearance features extracted from patch $l_j$ of image $x$ (\eg HOG features). Also let $\phi_d(l_j, \rootLocation)$ denote the deformation features of placing part $j$ at $l_j$ given that the root filter is placed at $\rootLocation$. We define the feature function $\phi(x, l_j, \rootLocation)=( \phi_a(x, l_j); \phi_d(l_j, \rootLocation) )$. For DPMs, we can rewrite Equation~\ref{eq:score_roots_dpm} as follows:
\begin{align}
	f_\beta(x, R) &= \max_{\rootLocation \in R} \max_{c=1}^k F_{c, 0} \cdot \phi_a(x, \rootLocation) \notag \\
		& \hspace{1.75cm} + \sum_{j=1}^\cntPartsPos \max_{l_j} w_{c, j} \cdot \phi(x, l_j, \rootLocation)
	\label{eq:score_roots_dpm_expanded}
\end{align}

In contrast, for GDPMs we have:
\begin{align}
	f_\gamma(x, R) &=  \max_{\rootLocation \in R} \max_{c=1}^k F_{c, 0} \cdot \phi(x, \rootLocation) \notag \\
		& \hspace{1.75cm} + \sum_{j=1}^\cntPartsPos \max_{l^+_j} w^+_{c, j} \cdot \phi(x, l^+_j, \rootLocation) \notag \\
		& \hspace{1.75cm} - \sum_{j=1}^\cntPartsNeg \max_{l^-_j} w^-_{c, j} \cdot \phi(x, l^-_j, \rootLocation) \label{eq:score_roots_gdpm_expanded}
\end{align}

One way to see that GDPM is more general than DPM is to note that the score function of Equation~\ref{eq:score_roots_dpm_expanded} is convex in the model parameters whereas Equation ~\ref{eq:score_roots_gdpm_expanded} is not.

\todo{mention that this is equivalent to doing max-min}

%-------------------------------------------------------------------------
\subsection{Training with Negative Parts}
We define the training objective of a GDPM as follows:
\begin{align}
	O(\gamma) =& \frac{1}{2} ||\gamma||^2 + C \sum_{i=1}^\cntExamples \max \{ 0, 1 - y_i f_\gamma(x_i, R_i) \} 
\label{eq:of_gdpm}
\end{align}
This objective function is non-convex. Moreover, unlike DPMs, fixing the latent variables for the foreground examples does \emph{not} make it convex. Thus, we cannot use Latent SVM framework to train GDPMs.

We deploy CCCP for training the objective function of Equation~\ref{eq:of_gdpm}. Recall that CCCP alternates between constructing a convex function that upper bounds the original objective function and optimizing the bound. 

We obtain a convex upper bound $B(\gamma)$ to the training objective by replacing $f_\gamma(x_i, R_i)$ with a convex upper bound $\check{f}_\gamma$ for background images and a concave lower bound $\hat{f}_\gamma$ for foreground images.
\begin{align}
	B(\gamma) =& \frac{1}{2} ||\gamma||^2 + C \sum_{\substack{i=1 \\ y_i=-1}}^\cntExamples \max \{ 0, 1 + \check{f}_\gamma(x_i, R_i) \} \notag \\
	& \hspace{0.9cm} + C \sum_{\substack{i=1 \\ y_i=+1}}^\cntExamples \max \{ 0, 1 - \hat{f}_\gamma(x_i, R_i) \}
	\label{eq:bound_gdpm}
\end{align}
In the rest of this section we first explain how the bounds are constructed and then elaborate on the optimization of the bound.

%-------------------------------------------------------------------------
\subsection{Constructing Convex Bounds}
In this section we explain how we obtain $\check{f}_\gamma$ and $\hat{f}_\gamma$ in order to construct the bound $B(\gamma)$ in Equation~\ref{eq:bound_gdpm}. Let $\gamma^*$ be the solution to the previous convex bound. We define $l^-_{i, j}(\rootLocation, c) = \argmax_l w^{*-}_{c, j} \cdot \phi(x_i, l, \rootLocation)$ to be the optimal placement of the $j$-th negative part using the previous model conditioned on the choice of the root location $\rootLocation$ and the mixture component $c$. 
We obtain $\check{f}_\gamma$ by fixing the placement of the negative parts according to $l^-_{i, j}(\rootLocation, c)$ as follows:
\begin{align}
	\check{f}_\gamma(x_i, R_i) &=  \max_{\rootLocation \in R} \max_{c=1}^k F_{c, 0} \cdot \phi(x_i, \rootLocation) \notag \\
		& \hspace{1.75cm} + \sum_{j=1}^\cntPartsPos \max_{l^+_j} w^+_{c, j} \cdot \phi(x_i, l^+_j, \rootLocation) \notag \\
		& \hspace{1.75cm} - \sum_{j=1}^\cntPartsNeg w^-_{c, j} \cdot \phi(x_i, l^-_{i, j}(\rootLocation, c), \rootLocation)
\end{align}
Let $(\rootLocation_i, c_i, l^+_i)$ denote the best placement of the root filter, choice of the mixture component, and placement of the positive parts using the model $\gamma^*$ given that the negative parts have been placed optimally according to $l^-_{i, j}(\rootLocation, c)$. We can formally define this as follows:
\begin{align}
	(\rootLocation_i, c_i, l^+_i) &= \argmax_{(\rootLocation, c, l)} F^*_{c, 0} \cdot \phi(x_i, \rootLocation) \notag \\
		& \hspace{1.75cm} + \sum_{j=1}^\cntPartsPos w^{*+}_{c, j} \cdot \phi(x_i, l_j, \rootLocation) \notag \\
		& \hspace{1.75cm} - \sum_{j=1}^\cntPartsNeg w^{*-}_{c, j} \cdot \phi(x_i, l^-_{i, j}(\rootLocation, c), \rootLocation)
\end{align}
We obtain $\hat{f}_\gamma$ as follows:
\begin{align}
	\hat{f}_\gamma(x_i, R_i) &= F_{c_i, 0} \cdot \phi(x_i, \rootLocation_i) \notag \\
		& \hspace{1.5cm} + \sum_{j=1}^\cntPartsPos w^+_{c_i, j} \cdot \phi(x_i, l^+_{i, j}, \rootLocation_i) \notag \\
		& \hspace{1.5cm} - \sum_{j=1}^\cntPartsNeg \max_{l^-_j} w^-_{c_i, j} \cdot \phi(x_i, l^-_j, \rootLocation_i)
\end{align}

\todo{explain that positive examples have max over locations for root filter}

%-------------------------------------------------------------------------
\todo{\subsection{Data mining}}
\todo{no notion of hard "negatives" any more! We have hard "examples" now!}

%-------------------------------------------------------------------------
\subsection{Initializing Negative Parts}
The positive parts in original DPM~\cite{FelzenszwalbMR08} is initialized by first learning a root filter (whole object detector without parts). Then in order to initialize the location and weights of a part filter, a submatrix of root filter is sought which has the maximal positive energy. Positive energy is measured by sum of squared \textit{positive} weights in the submatrix of the root filter. The first part is initialized with the best submatrix location and weights. Then all the weights are zeroed at that location and the procedure is repeated to initialize a second part. This continues until the desired number of parts are added. We initialize positive parts in the same manner. Also, we initialize the negative part similarly, except that we try to find the submatrix with highest negative energy being sum of squared \textit{negative} weights of the submatrix. This involves the main results of the paper.\\
We further initialize the negative parts with the positive parts of similar classes. Particularly, we initialize the negative parts for \textit{cow} GDPM model by taking positive parts from \textit{horse} DPM model.
%-------------------------------------------------------------------------
\subsection{Inference for Data Mining}
When doing inference for GDPM data mining, we need to construct a concave lower bound for positive samples and convex upper bound for negative samples. That is, we need to fix the position of negative parts for negative samples at the location of relabeling. We further need to fix the location of positive parts, mixture component and root filter location for positive samples to the assignments at the relabeling. On the other hand, the positve parts and mixture component needs to be maximized for negative samples and negative parts needs to be updated for positive samples. Storing the fixed values of latent variables for all negative samples (hundreds of thousands negative bounding box for each image) is prohibitively memory-consuming. Thus, in our implementation, we do the following. At each relabeling step we keep a copy of the model. We also store the inferred component and location of the root filter only for positive samples (requires low amount of memory since number of positive annotations are usually low). Then at each iteration of data mining: For positive samples we take the current model and roll back the positive parts to the copied model, and do the inference at the saved location and with the saved component. As for negative examples, we take the current model and roll back the negative parts to the copied model and do the inference. This way we simply take care of convex upper bound and concave lower bounds with low memory footprint. However, this comes at the cost of two times more computational complexity. Since the main complexity of the inferences goes back to convolution of part/root filters, the remedy for this would be to save the output of convolution for positive parts on positive examples and negative parts on negative examples (proportional to the number of images and independent of number of negative bounding boxes per image).


==> Dataset.tex <==
\section{Dataset}
\label{sec:dataset}
Random images from Cat Head dataset \cite{Parkhi12a}. Note that, many of the cat heads are not frontal.
\begin{figure}[h!]
	\begin{subfigure}{0.5\textwidth}
	\includegraphics[trim = 0mm 0mm 0mm 0mm, clip,width=0.22\linewidth]{images/dataset/Abyssinian_1.jpg}
	\includegraphics[trim = 0mm 0mm 0mm 0mm, clip,width=0.22\linewidth]{images/dataset/Abyssinian_2.jpg}
	\includegraphics[trim = 0mm 0mm 0mm 0mm, clip,width=0.22\linewidth]{images/dataset/Abyssinian_3.jpg}
	\includegraphics[trim = 0mm 0mm 0mm 0mm, clip,width=0.22\linewidth]{images/dataset/Abyssinian_4.jpg}
	\caption{Abyssinian}
	\label{ab}
	\end{subfigure}
	\begin{subfigure}{0.5\textwidth}
	\includegraphics[trim = 0mm 0mm 0mm 0mm, clip,width=0.22\linewidth]{images/dataset/Bengal_1.jpg}
	\includegraphics[trim = 0mm 0mm 0mm 0mm, clip,width=0.22\linewidth]{images/dataset/Bengal_2.jpg}
	\includegraphics[trim = 0mm 0mm 0mm 0mm, clip,width=0.22\linewidth]{images/dataset/Bengal_3.jpg}
	\includegraphics[trim = 0mm 0mm 0mm 0mm, clip,width=0.22\linewidth]{images/dataset/Bengal_4.jpg}
	\caption{Bengal}
	\label{ab}
	\end{subfigure}\\
	\begin{subfigure}{0.5\textwidth}
	\includegraphics[trim = 0mm 0mm 0mm 0mm, clip,width=0.22\linewidth]{images/dataset/Birman_1.jpg}
	\includegraphics[trim = 0mm 0mm 0mm 0mm, clip,width=0.22\linewidth]{images/dataset/Birman_2.jpg}
	\includegraphics[trim = 0mm 0mm 0mm 0mm, clip,width=0.22\linewidth]{images/dataset/Birman_3.jpg}
	\includegraphics[trim = 0mm 0mm 0mm 0mm, clip,width=0.22\linewidth]{images/dataset/Birman_4.jpg}
	\caption{Birman}
	\label{ab}
	\end{subfigure}
	\begin{subfigure}{0.5\textwidth}
	\includegraphics[trim = 0mm 0mm 0mm 0mm, clip,width=0.22\linewidth]{images/dataset/Bombay_1.jpg}
	\includegraphics[trim = 0mm 0mm 0mm 0mm, clip,width=0.22\linewidth]{images/dataset/Bombay_2.jpg}
	\includegraphics[trim = 0mm 0mm 0mm 0mm, clip,width=0.22\linewidth]{images/dataset/Bombay_3.jpg}
	\includegraphics[trim = 0mm 0mm 0mm 0mm, clip,width=0.22\linewidth]{images/dataset/Bombay_4.jpg}
	\caption{Bombay}
	\label{ab}
	\end{subfigure}\\	
	\begin{subfigure}{0.5\textwidth}
	\includegraphics[trim = 0mm 0mm 0mm 0mm, clip,width=0.22\linewidth]{images/dataset/British_Shorthair_1.jpg}
	\includegraphics[trim = 0mm 0mm 0mm 0mm, clip,width=0.22\linewidth]{images/dataset/British_Shorthair_2.jpg}
	\includegraphics[trim = 0mm 0mm 0mm 0mm, clip,width=0.22\linewidth]{images/dataset/British_Shorthair_3.jpg}
	\includegraphics[trim = 0mm 0mm 0mm 0mm, clip,width=0.22\linewidth]{images/dataset/British_Shorthair_4.jpg}
	\caption{British Shorthair}
	\label{ab}
	\end{subfigure}
	\begin{subfigure}{0.5\textwidth}
	\includegraphics[trim = 0mm 0mm 0mm 0mm, clip,width=0.22\linewidth]{images/dataset/Egyptian_Mau_1.jpg}
	\includegraphics[trim = 0mm 0mm 0mm 0mm, clip,width=0.22\linewidth]{images/dataset/Egyptian_Mau_2.jpg}
	\includegraphics[trim = 0mm 0mm 0mm 0mm, clip,width=0.22\linewidth]{images/dataset/Egyptian_Mau_3.jpg}
	\includegraphics[trim = 0mm 0mm 0mm 0mm, clip,width=0.22\linewidth]{images/dataset/Egyptian_Mau_4.jpg}
	\caption{Egyptian Mau}
	\label{ab}
	\end{subfigure}\\	
	\begin{subfigure}{0.5\textwidth}
	\includegraphics[trim = 0mm 0mm 0mm 0mm, clip,width=0.22\linewidth]{images/dataset/Maine_Coon_1.jpg}
	\includegraphics[trim = 0mm 0mm 0mm 0mm, clip,width=0.22\linewidth]{images/dataset/Maine_Coon_2.jpg}
	\includegraphics[trim = 0mm 0mm 0mm 0mm, clip,width=0.22\linewidth]{images/dataset/Maine_Coon_3.jpg}
	\includegraphics[trim = 0mm 0mm 0mm 0mm, clip,width=0.22\linewidth]{images/dataset/Maine_Coon_4.jpg}
	\caption{Maine Coon}
	\label{ab}
	\end{subfigure}
	\begin{subfigure}{0.5\textwidth}
	\includegraphics[trim = 0mm 0mm 0mm 0mm, clip,width=0.22\linewidth]{images/dataset/Persian_1.jpg}
	\includegraphics[trim = 0mm 0mm 0mm 0mm, clip,width=0.22\linewidth]{images/dataset/Persian_2.jpg}
	\includegraphics[trim = 0mm 0mm 0mm 0mm, clip,width=0.22\linewidth]{images/dataset/Persian_3.jpg}
	\includegraphics[trim = 0mm 0mm 0mm 0mm, clip,width=0.22\linewidth]{images/dataset/Persian_4.jpg}
	\caption{Persian}
	\label{ab}
	\end{subfigure}\\	
	\begin{subfigure}{0.5\textwidth}
	\includegraphics[trim = 0mm 0mm 0mm 0mm, clip,width=0.22\linewidth]{images/dataset/Ragdoll_1.jpg}
	\includegraphics[trim = 0mm 0mm 0mm 0mm, clip,width=0.22\linewidth]{images/dataset/Ragdoll_2.jpg}
	\includegraphics[trim = 0mm 0mm 0mm 0mm, clip,width=0.22\linewidth]{images/dataset/Ragdoll_3.jpg}
	\includegraphics[trim = 0mm 0mm 0mm 0mm, clip,width=0.22\linewidth]{images/dataset/Ragdoll_4.jpg}
	\caption{Ragdoll}
	\label{ab}
	\end{subfigure}
	\begin{subfigure}{0.5\textwidth}
	\includegraphics[trim = 0mm 0mm 0mm 0mm, clip,width=0.22\linewidth]{images/dataset/Russian_Blue_1.jpg}
	\includegraphics[trim = 0mm 0mm 0mm 0mm, clip,width=0.22\linewidth]{images/dataset/Russian_Blue_2.jpg}
	\includegraphics[trim = 0mm 0mm 0mm 0mm, clip,width=0.22\linewidth]{images/dataset/Russian_Blue_3.jpg}
	\includegraphics[trim = 0mm 0mm 0mm 0mm, clip,width=0.22\linewidth]{images/dataset/Russian_Blue_4.jpg}
	\caption{Russian Blue}
	\label{ab}
	\end{subfigure}\\
	\begin{subfigure}{0.5\textwidth}
	\includegraphics[trim = 0mm 0mm 0mm 0mm, clip,width=0.22\linewidth]{images/dataset/Siamese_1.jpg}
	\includegraphics[trim = 0mm 0mm 0mm 0mm, clip,width=0.22\linewidth]{images/dataset/Siamese_2.jpg}
	\includegraphics[trim = 0mm 0mm 0mm 0mm, clip,width=0.22\linewidth]{images/dataset/Siamese_3.jpg}
	\includegraphics[trim = 0mm 0mm 0mm 0mm, clip,width=0.22\linewidth]{images/dataset/Siamese_4.jpg}
	\caption{Siamese}
	\label{ab}
	\end{subfigure}
	\begin{subfigure}{0.5\textwidth}
	\includegraphics[trim = 0mm 0mm 0mm 0mm, clip,width=0.22\linewidth]{images/dataset/Sphynx_1.jpg}
	\includegraphics[trim = 0mm 0mm 0mm 0mm, clip,width=0.22\linewidth]{images/dataset/Sphynx_2.jpg}
	\includegraphics[trim = 0mm 0mm 0mm 0mm, clip,width=0.22\linewidth]{images/dataset/Sphynx_3.jpg}
	\includegraphics[trim = 0mm 0mm 0mm 0mm, clip,width=0.22\linewidth]{images/dataset/Sphynx_4.jpg}
	\caption{Sphynx}
	\label{ab}
	\end{subfigure}\\	
	\caption{Samples of Pet~\cite{Parkhi12a} dataset used for cat head detection}
	\label{tab:voc}
\end{figure}

==> Dependency.tex <==
\section{Dependency Structure}
\label{sec:dependency}
\noindent Complexity of evaluating GLVM scoring function %(Equation~\ref{eq:GLVM_score3}) 
is governed by the dependency structure of the underlying feature function $\phi$. In the most extreme case, with no independence assumption at all, evaluating the scoring function would require exhaustive search on the space of all possible assignments of the latent variables. This grows exponentially with the number of latent variables and becomes intractable very quickly. \\
\noindent Tree-structured dependencies are particularly interesting and widely used in practice~\cite{FelzenszwalbMR08,AzizpourL12}. Complexity of evaluating the scoring function with tree-structured dependency is quadratic in the cardinality of the domain of a single latent variable. \\
\noindent Dependency structure of the feature function also affects the complexity of finding the fixed latent assignments in %Equations ~\ref{eq:fixed_negative_parts} and~\ref{eq:fixed_positive_parts}
inference functions of training, and hence, the construction of the bounds $B_t$. \\
Another note is that although we call $\lv{+}{k}{}$s positive latent variables and $\lv{-}{k}{}$s negative latent variables, this is only for simplicity of notation and explanations. That is, the true meaning of these variables as evidences or counter evidences for the positive class changes by the dependency structure of the scoring function. For example a negative latent variable depending on another negative latent variable of the positive class is not a counter evidence for positive class nor is a evidence. Conversely, positive latent variables dependent to a negative latent variable act as a counter evidence for the positive class. 
\todo{Explain what happens to the interpretation of $z^{+}$ and $z^{-}$ as for the original class in different branches and when having loops}\\


==> Hough.tex <==
\section{Show Case 2: Latent Hough  Transform}
\label{sec:hough}
Hough transform (HT), in computer vision, has been used as a non-parametric voting scheme to localize objects. In Implicit Shape Models \cite{LeibeLS08}, the score of an object hypothesis (image, location, scale, etc.) on a query image is calculated using a codebook $C$ of evidences $c_i$. Each evidence votes in favor of the hypothesis proportional to the number of training images $x_j$ in agreement with the hypothesis. Formally, the score of a hypothesis $h$ is calculated as below,
\mathenv{
S(h) = \sum_i s(h|c_i),   \qquad\qquad\quad  s(h|c_i) = \sum_j s(h|c_i,x_j)
\label{HT_score}
}
where $s(h|c_i)$ accumulates, over all positive training images $x_j$, if (or to what extent) hypothesis $h$ agrees with the positive image based on evidence $c_i$. The agreement, $s(h|c_i,x_j)$, is usually measured as how similar is the relative position of the evidence to the hypothesis on query image and to the ground truth on positive image $x_j$.  The codebook of evidences is constructed by clustering several patches extracted from \textit{positive} regions. \\
HT has been shown to be tolerant to certain levels of deformation and thanks to its simple non-parametric nature can be widely applied to many computer vision tasks (from edge detection to object segmentation). However, one of the main issues with HT is its susceptibility to aggregation of inconsistent evidences. For instance, evidences of different viewpoints of cars can accidentally co-vote for a specific hypothesis. This increases the false positive rate of HT systems and is unwanted. Razavi \etal \cite{RazaviGKG12} alleviates this issue by introducing latent Hough transform (LHT). LHT models grouping of consistent evidences together using latent variable as below,
\mathenv{
&S(h) = \max_{z\in\{1...Z\}} w^{T}\phi(h,z) \footnotemark\\
&\phi(h,z) = (\mathbf{\emptyset}^{(z-1) \times |C|},s(h|c_1),s(h|c_2),...,s(h|c_{|C|}),\emptyset^{(Z-z) \times |C|})
\label{LHT_phi}
}
\footnotetext{Note that our notation is in vector form and slightly differs from \cite{RazaviGKG12} in a way that it complies to our formulations in previous sections.}
where $\emptyset^{n}$ indicates a zero vector of length $n$. LHT achieved significant improvements over HT by reducing the false positive rate \cite{RazaviGKG12}.\\
In order to reformulate the problem as a GLVM, we need to introduce negative evidences to cast negative votes in the scoring function of HT. Interestingly, the notion of negative voting has been introduced back in 1983 \cite{Brown83}. Essentially, the new HT scoring function with negative votings looks as follows,
\mathenv{
S(h) = \sum_{c^{+}_i\in C^+} s(h|c^{+}_i) - \sum_{c^{-}_i\in C^-} s(h|c^{-}_i)
\label{NHT_score}
}
where codebook $C^+$ is generated as before, on positive samples, but on the other hand codebook $C^-$ is generated over (hard) negative samples. \cite{Brown83} showed that negative voting helps to reduce the unwanted bias to the positive training set. However the distribution of the negative class is extremely more multi-modal than the positive class (any classes except positive class generates negative samples). That increases the error (false negative rate) of using Equation \ref{NHT_score} instead of Equation \ref{HT_score} due to the aggregation of inconsistent negative evidences. That can explain the reason why negative voting is not popular for HT based object recognition. However, the GLVM framwork proposed in this work can potentially solve this problem by grouping the negatives into consistent groups as LHT does for positive evidences. The corresponding GLVM will then be defined as,
\mathenv{
&S(h) = \max_{z^+\in\{1...Z^+\}} w^{T}\phi^+(h,z^+) - \max_{z^-\in\{1...Z^-\}} w^{T}\phi^-(h,z^-)
}
$\phi^+$ and $\phi^-$ is defined same as Equation \ref{LHT_phi} with $s(h|c_i)$ substituted by $s(h|c^{+}_i)$ and $s(h|c^{-}_i)$ respectively. \\
It should be noted the GLVM version of HT can make use of the negative data in a significantly more effective way. It's also worth mentioning that the construction of the negative codebook will be more effective if is done on a \textit{hard negative} set of a regular HT system. For instance, assuming the task of car detection, many of the hard negatives would belong to other wheeled vehicles such as bike, motorbike, bus, train, etc. which could be used for the construction of negative evidence and subsequently latent grouping of those negative evidences.


==> Intuition.tex <==
\vspace{-0.35cm}
\section{Intuitive example of LVM and GLVM}
\vspace{0cm}
Figure \ref{fig:intuition} gives intuitive examples of positive and negative latent variables.
\begin{figure}[h!]
\centering
\includegraphics[trim=1.6cm 5.3cm 9cm 1cm, clip=true, width=1\linewidth]{images/LVM_vs_GLVM_Example.pdf}
\caption{\textbf{Intuitive example of LVM and GLVM.} Assume the task of \textit{cow} image classfication. This figure visualizes examples of possible latent variables for LVM and GLVM models. A latent variable can be assigned at image level such as the background scene and then gradually go down a hierarchy of objects, parts and subparts. Positive latent variables (modeling evidences for cow) of an LVM may correspond to different scenes where cow is likely to be seen \eg stable, meadow (blue boxes in the first column). Another positive latent variable can be assigned to the location of the cow in the image (second column, first row). In addition, location of different parts of cow \eg head, back, legs can be modeled as other latent variables dependent to the latent variable of cow location (top right). All these examples of latent variables in LVMs look for evidences for the existence of cow. In GLVM we encourage the modeling of counter evidences through negative latent variables. For example at high level a negative latent variable may correspond to scenes where cow is unlikely to be found \eg office, laundromat, or airport (bottom left). Meadow is an evidence for cow, but cows are less likely to be seen in a meadow beside camping tents (a dependent negative latent variable to positive latent variable meadow). Horses are visually similar to cow but people usually do not ride cows thus a human on top of cow can be negative evidence (a negative latent variable dependent to the positive latent variable of cow location). Furthermore, human, a negative latent variable for cow, can have its own positive latent variable as parts \eg face and shoulders (bottom right).}
\label{fig:intuition}
\end{figure}

==> Results.tex <==
\section{Precision Recall Curves}
\label{sec:PR}
In this section, the precision recall curves for DPM comparing with its best performing GDPM variant is plotted for animals subset of PASCAL VOC 2007. For the class of \textit{cow} an extra curve is plotted which belongs to a different initialization of negative parts using \textit{horse} DPM model. For the class of \textit{bird} and \textit{dog} while the AP (calculated by average of 11 sampled points) is equal for GDPM and DPM, the GDPM curve shows slightly better precision at lower recalls.
\begin{figure}[h!]
    \begin{subfigure}{.45\textwidth}
    \centering
    		\includegraphics[trim = 13mm 0mm 30mm 0mm, clip,width=1\linewidth]{images/CowInit_PR.pdf}
    		\vspace{-0.2cm}
            \caption{PR curve for \textit{cow} in PASCAL VOC 2007 using original DPM, GDPM with 2 negative parts, and GDPM with one negative part initialized by horse DPM model.}
            \label{fig:cowPR}
	\end{subfigure}
	\qquad
    \begin{subfigure}{.45\textwidth}
    \vspace{0.7cm}
    \centering
    		\includegraphics[trim = 13mm 0mm 30mm 0mm, clip,width=1\linewidth]{images/Bird_PR.pdf}
    		\vspace{-0.2cm}
            \caption{PR curve for \textit{bird} in PASCAL VOC 2007 using original DPM, GDPM with 1 negative part. Although the AP (computed by taking average of 10 sampled points from the curve) is equal, the GDPM curve has slightly higher precision at lower recall.}
            \label{fig:cowPR}
	\end{subfigure}\\
    \begin{subfigure}{.45\textwidth}
    \vspace{1.1cm}
    \centering
    		\includegraphics[trim = 13mm 0mm 30mm 0mm, clip,width=1\linewidth]{images/Dog_PR.pdf}
    		\vspace{-0.2cm}
            \caption{PR curve for \textit{dog} in PASCAL VOC 2007 using original DPM, GDPM with 1 negative part. Although the AP (computed by taking average of 10 sampled points from the curve) is equal, the GDPM curve has slightly higher precision at lower recall.}
            \label{fig:cowPR}
	\end{subfigure}
	\qquad
    \begin{subfigure}{.45\textwidth}
    \vspace{0.3cm}
    \centering
    		\includegraphics[trim = 13mm 0mm 30mm 0mm, clip,width=1\linewidth]{images/Sheep_PR.pdf}
    		\vspace{-0.2cm}
            \caption{PR curve for \textit{sheep} in PASCAL VOC 2007 using original DPM, GDPM with 2 negative part. The GDPM curve exhibits higher precision at different recalls.}
            \label{fig:cowPR}
	\end{subfigure}\\
	\caption{PR curves for animals subset of PASCAL VOC 2007}
	\label{fig:PR}
\end{figure}

==> Weights.tex <==
\section{Negative Weights v.s. Negative Latent Variables}
\label{sec:weights}

\todo{Linear models ($w'\phi$) can have negative weights for positive latent variables, here we describe what is the conceptual difference between those negative weights and the positive weights of negative latent variables, give intuitive examples!}

==> alg1.tex <==
\begin{algorithm}[h]
\footnotesize
	\begin{algorithmic} % [1]
	\caption{Training GLVM classifiers. \quad \scriptsize Note that equation numbers refer to the main paper.}
		\INPUT{$D=\{(x_i,y_i)\}_{i=1}^n, w_0$}
		\STATE $t\gets 0$
		\REPEAT 
		\STATE Construct $\check{S}_t(w)$ from Equation (11) and $w_t$
		\STATE Construct $\hat{S}_t(w)$ from Equation (12) and $w_t$
		\STATE Construct $B_t(w)$ from Equation (8)
		\STATE $w_{t+1} \gets \argmin_w B_t(w)$
		\STATE $t\gets t+1$
		\UNTIL{$w_t$ does not change}
		\OUTPUT $w_t$\\
	%\caption{as}
	\label{alg:training}
	\end{algorithmic}
	%\label{alg:training}
\vspace{-0.3cm}
\end{algorithm}
%      \begin{algorithmic}
%        \WHILE{$N \neq 0$}
%          \IF{$N$ is even}
%            \STATE $X \Leftarrow X \times X$
%            \STATE $N \Leftarrow N / 2$
%          \ENDIF
%        \ENDWHILE
%      \end{algorithmic}

==> alg_table.tex <==

\input{table2.tex}

